Stochastic Reweighted Gradient Descent

Despite the strong theoretical guarantees that variance-reduced finite-sum optimization algorithms enjoy, their applicability remains limited to cases where the memory overhead they introduce (SAG/SAGA), or the periodic full gradient computation they require (SVRG/SARAH) are manageable. A promising approach to achieving variance reduction while avoiding these drawbacks is the use of importance sampling instead of control variates. While many such methods have been proposed in the literature, directly proving that they improve the convergence of the resulting optimization algorithm has remained elusive. In this work, we propose an importance-sampling-based algorithm we call SRG (stochastic reweighted gradient). We analyze the convergence of SRG in the strongly-convex case and show that, while it does not recover the linear rate of control variates methods, it provably outperforms SGD. We pay particular attention to the time and memory overhead of our proposed method, and design a specialized red-black tree allowing its efficient implementation. Finally, we present empirical results to support our findings.

==> appendices/review_sgd.tex <==
Before we give the proofs of the main results
that study the convergence of SRG, we review here
the standard analysis of SGD. This will allow
us to compare the performance of SGD and SRG.
Recall that SGD uses the following recurrence relation:
\begin{equation}
    x_{k+1} = x_k - \alpha_k \nabla f_{i_k}(x_k)
    \label{SGD}
\end{equation}
where $i_k$ is uniformly distributed on $[n]$.

The main result of the analysis of SGD is the following
Theorem:
\begin{theorem}
    Suppose that Assumptions \ref{strongly-convex},
    \ref{convex}, and \ref{smooth} hold,
    and that $x_k$ evolves according to (\ref{SGD})
    with $\alpha_k \leq 1/2L$.
    Then:
    \begin{equation*}
        \E{\sqnorm{x_{k+1} - \xstar}} \leq 
        (1-\alpha_k\mu) \E{\sqnorm{x_k - \xstar}} + 2 \alpha_k^2 \sigma^2
    \end{equation*}
    \label{sgd_one_step}
\end{theorem}
\begin{proof}
    Taking expectation with respect to $i_k$ conditional on $(i_t)_{t=1}^{k-1}$
    we have:
    \begin{align*}
        &\E{\sqnorm{x_{k+1} - \xstar}} \\
        &= \E{\sqnorm{x_{k} - \alpha_k \nabla f_{i_k}(x_k) - \xstar}} \\
        &= \sqnorm{x_k - \xstar} - 
        2 \alpha_k \inp{\E{\nabla f_{i_k}(x_k)}}{x_k - \xstar} +
        \alpha_k^2 \E{\sqnorm{\nabla f_{i_k}(x_k)}} \\
        &\leq \sqnorm{x_k - \xstar} -
        2 \alpha_k \inp{\nabla F(x_k)}{x_k - \xstar} +
        2 \alpha_k^2 \E{\sqnorm{\nabla f_{i_k}(x_k) - \nabla f_{i_k}(\xstar)}} +
        2 \alpha_k^2 \E{\sqnorm{\nabla f_{i_k}(\xstar)}} \\
        &\leq (1 - \alpha_k\mu) \sqnorm{x_k - \xstar} +
        2 \alpha_k^2 \sigma^2 +
        2 \alpha_k \left(2L\alpha_k - 1\right) \left[F(x_k) - F(\xstar)\right]
    \end{align*}
    where the fourth line follows from Proposition \ref{youngs_inequality},
    and the fifth line from the definition of $\sigma^2$ in
    section \ref{convergence}, Assumption \ref{strongly-convex}
    (strong-convexity of F) applied to the inner product term,
    and Lemma \ref{grad_norm_bound} applied to the remaining term.
    For $\alpha_k \leq 1/2L$ the third term is negative, so
    that taking total expectation on both sides yields the result.
\end{proof}

The above Theorem leads to the following convergence
rate for SGD with a constant step size.
\begin{corollary}
    Under the assumptions of Theorem \ref{sgd_one_step},
    and using a constant step size $\alpha \leq 1/2L$,
    we have for any $k \in \mathbb{N}$:
    \begin{equation*}
        \E{\sqnorm{x_k - \xstar}} \leq 
        (1 - \alpha \mu)^k \sqnorm{x_0 - \xstar}
        +
        \frac{2\alpha \sigma^2}{\mu}
    \end{equation*}
\end{corollary}
\begin{proof}
    Starting from $\sqnorm{x_k - \xstar}$ and alternating
    taking expectation and applying Theorem \ref{sgd_one_step}
    we get:
    \begin{align*}
        \E{\sqnorm{x_k - \xstar}} 
        &\leq
        (1-\alpha \mu)^k \sqnorm{x_0 - \xstar}
        + 2\alpha^2 \sigma^2 \sum_{t=0}^{k-1} (1-\alpha\mu)^t \\
        &\leq
        (1 - \alpha\mu)^k \sqnorm{x_0 - \xstar}
        + 2\alpha^2 \sigma^2 \sum_{t=0}^{\infty} (1-\alpha\mu)^t \\
        &= (1 - \alpha\mu)^k \sqnorm{x_0 - \xstar}
        + \frac{2\alpha\sigma^2}{\mu}
    \end{align*}
\end{proof}

For decreasing step sizes, we have the following result:
\begin{corollary}
    Under the assumptions of Theorem \ref{sgd_one_step},
    and using the step sizes:
    \begin{equation*}
        \alpha_k = \frac{2(k + k_0) + 1}
        {\left[c + (k+k_0)(k+k_0+2)\right]\mu}
    \end{equation*}
    where:
    \begin{align*}
        k_0 &= \frac{4L}{\mu} - 2 \\
        c &= \frac{2L}{\mu}
    \end{align*}
    Then:
    \begin{equation*}
        \E{\sqnorm{x_k - \xstar}}
        \leq O\left(\frac{\sqnorm{x_0 - \xstar}}{k^2}\right) +
        O\left(\frac{\sigma^2}{k}\right)
    \end{equation*}
\end{corollary}
\begin{proof}
    It is easy to check that $\alpha_0 = 1/2L$,
    and that the sequence $(\alpha_k)_{k=1}^{\infty}$
    is decreasing, so that the step size condition
    of Theorem \ref{sgd_one_step} holds for
    all $k \in \mathbb{N}$. Fix $k \in \mathbb{N}$.
    We have by Theorem \ref{sgd_one_step} for any
    $t \in [k-1]\cup \{0\}$:
    \begin{align*}
        \E{\sqnorm{x_{t+1} - \xstar}} &\leq 
        (1-\alpha_t\mu) \E{\sqnorm{x_{t} - \xstar}} + 
        2\alpha_t^2 \sigma^2 \\[1em]
        &= \frac{c + (t+k_0-1)(t+k_0+1)}{c + (t+k_0)(t+k_0+2)} 
        \E{\sqnorm{x_t - \xstar}}
        + 2\alpha_t^2 \sigma^2
    \end{align*}
    multiplying both sides by \(\left[c + (t+k_0)(t+k_0+2)\right]\) and
    noticing that:
    \begin{equation*}
        \left[c + (t+k_0)(t+k_0+2)\right]\alpha_t^2 = 
        \frac{\left[2 (t + k_0) + 1\right]^2}
        {\left[c + (t+k_0)(t+k_0+2)\right]} \leq 4
    \end{equation*}
    we get:
    \begin{align*}
        \left[c + (t+k_0)(t+k_0+2)\right]\E{\sqnorm{x_{t+1} - \xstar}} - 
        \left[c + (t+k_0-1)(t+k_0+1)\right]\E{\sqnorm{x_{t} - \xstar}}
        \leq 8\sigma_*^2
    \end{align*}
    summing the \(k\) inequalities for \(t \in [k-1] \cup \{0\}\) and noticing
    that the left side is a telescoping sum we obtain:
    \begin{align*}
        \left[c + (k+k_0)(k+k_0+2)\right]\E{\sqnorm{x_k - \xstar}}
        -
        \left[c + (k_0 - 1)(k_0 + 1)\right] \sqnorm{x_0 - \xstar}
        \leq 
        8k\sigma^2
    \end{align*}
    rearranging yields:
    \begin{align*}
        \E{\sqnorm{x_k - \xstar}} \leq 
        \frac{c + (k_0 - 1)(k_0 + 1)}{c + (k+k_0)(k+k_0+2)}
        \sqnorm{x_0 - \xstar} +
        \frac{8k\sigma^2}{c + (k+k_0)(k+k_0+2)}
    \end{align*}
\end{proof}
